Trust Driven On-Demand Scheme for Client Deployment in Federated Learning

Containerization technology plays a crucial role in Federated Learning (FL) setups, expanding the pool of potential clients and ensuring the availability of specific subsets for each learning iteration. However, doubts arise about the trustworthiness of devices deployed as clients in FL scenarios, especially when container deployment processes are involved. Addressing these challenges is important, particularly in managing potentially malicious clients capable of disrupting the learning process or compromising the entire model. In our research, we are motivated to integrate a trust element into the client selection and model deployment processes within our system architecture. This is a feature lacking in the initial client selection and deployment mechanism of the On-Demand architecture. We introduce a trust mechanism, named "Trusted-On-Demand-FL", which establishes a relationship of trust between the server and the pool of eligible clients. Utilizing Docker in our deployment strategy enables us to monitor and validate participant actions effectively, ensuring strict adherence to agreed-upon protocols while strengthening defenses against unauthorized data access or tampering. Our simulations rely on a continuous user behavior dataset, deploying an optimization model powered by a genetic algorithm to efficiently select clients for participation. By assigning trust values to individual clients and dynamically adjusting these values, combined with penalizing malicious clients through decreased trust scores, our proposed framework identifies and isolates harmful clients. This approach not only reduces disruptions to regular rounds but also minimizes instances of round dismissal, Consequently enhancing both system stability and security.

==> cas-refs.tex <==

@misc{Googlecluster,
  author = {Google},
  title = {Google Cluster Workload Traces},
  year = {2019},
  publisher = {Google},
  journal = {Google Research},
  howpublished = {\url{https://research.google/tools/datasets/google-cluster-workload-traces-2019/}}
}

@InProceedings{randomm,
  title = 	 {{Communication-Efficient Learning of Deep Networks from Decentralized Data}},
  author = 	 {McMahan, Brendan and Moore, Eider and Ramage, Daniel and Hampson, Seth and Arcas, Blaise Aguera y},
  booktitle = 	 {Proceedings of the 20th International Conference on Artificial Intelligence and Statistics},
  pages = 	 {1273--1282},
  year = 	 {2017},
  editor = 	 {Singh, Aarti and Zhu, Jerry},
  volume = 	 {54},
  series = 	 {Proceedings of Machine Learning Research},
  month = 	 {20--22 Apr},
  publisher =    {PMLR},
  pdf = 	 {http://proceedings.mlr.press/v54/mcmahan17a/mcmahan17a.pdf},
  url = 	 {https://proceedings.mlr.press/v54/mcmahan17a.html}
}



@article{neuraln,
author = {Yuan, Xiaoyong and He, Pan and Zhu, Qile and Li, Xiaolin},
year = {2019},
month = {01},
pages = {1-20},
title = {Adversarial Examples: Attacks and Defenses for Deep Learning},
volume = {PP},
journal = {IEEE Transactions on Neural Networks and Learning Systems},
doi = {10.1109/TNNLS.2018.2886017}
}

@ARTICLE{halaa,  author={Shamseddine, Hala and Nizam, Jana and Hammoud, Ahmad and Mourad, Azzam and Otrok, Hadi and Harmanani, Haidar and Dziong, Zbigniew},  journal={IEEE Network},   title={A Novel Federated Fog Architecture Embedding Intelligent Formation},   year={2021},  volume={35},  number={3},  pages={198-204},  doi={10.1109/MNET.011.2000505}}

@BOOK{GA,
  TITLE = {An Introduction to Genetic Algorithms},
  AUTHOR = {Mitchell, Melanie},
  YEAR = {1996},
  PUBLISHER = {MA: MIT Press, ISBN 9780585030944},
}
@article{knapsack,
author = {Adamuthe, Amol and Sale, Vaishnavi and Mane, Sandeep},
year = {2020},
month = {01},
pages = {160-167},
title = {Solving single and multi-objective 01 Knapsack Problem using Harmony Search Algorithm},
volume = {64},
journal = {Journal of scientific research},
doi = {10.37398/JSR.2020.640136}
}

@article{hihi,
title = "Pareto set approximation by the method of adjustable weights and successive lexicographic goal programming",
author = "Pardalos, {Panos M} and Ingrida Steponavice and Antanas Zilinskas",
year = "2012",
doi = "10.1007/s11590-011-0291-5",
language = "English",
volume = "6",
pages = "665 -- 678",
journal = "Optimization Letters",
issn = "1862-4472",
publisher = "Springer-Verlag London Ltd.",
number = "4",
}
%1 
@ARTICLE{mario1,  author={Sami, Hani and Mourad, Azzam},  journal={IEEE Transactions on Network and Service Management},   title={Dynamic On-Demand Fog Formation Offering On-the-Fly IoT Service Deployment},   year={2020},  volume={17},  number={2},  pages={1026-1039},  doi={10.1109/TNSM.2019.2963643}}

%2
@ARTICLE{mario2,  author={Sami, Hani and Mourad, Azzam and El-Hajj, Wassim},  journal={IEEE/ACM Transactions on Networking},   title={Vehicular-OBUs-As-On-Demand-Fogs: Resource and Context Aware Deployment of Containerized Micro-Services},   year={2020},  volume={28},  number={2},  pages={778-790},  doi={10.1109/TNET.2020.2973800}}


%3
@inproceedings{mario3,
author = {Nishio, Takayuki and Yonetani, Ryo},
year = {2019},
month = {05},
pages = {1-7},
title = {Client Selection for Federated Learning with Heterogeneous Resources in Mobile Edge},
doi = {10.1109/ICC.2019.8761315}
}

%3
@inproceedings{mario4,
title={Diverse Client Selection for Federated Learning via Submodular Maximization},
author={Ravikumar Balakrishnan and Tian Li and Tianyi Zhou and Nageen Himayat and Virginia Smith and Jeff Bilmes},
booktitle={International Conference on Learning Representations},
year={2022},
url={https://openreview.net/forum?id=nwKXyFvaUm}
}

%3
@ARTICLE{mario5,
  author    = {J. Xu and H. Wang},
  title     = {Client selection and bandwidth allocation in wireless federated learning networks: A long-term perspective},
  journal   = {IEEE Tran.sWireless Commun},
  volume    = 20,
  number    = 2,
  pages     = {1188–1200},
  month     = {Feb},
  year      = 2021,
}



%3
@ARTICLE{mario6,  author={Yu, Liangkun and Albelaihi, Rana and Sun, Xiang and Ansari, Nirwan and Devetsikiotis, Michael},  journal={IEEE Internet of Things Journal},   title={Jointly Optimizing Client Selection and Resource Management in Wireless Federated Learning for Internet of Things},   year={2022},  volume={9},  number={6},  pages={4385-4395},  doi={10.1109/JIOT.2021.3103715}}

%3
@ARTICLE{mario7,
  author    = {J. Yao and N. Ansari},
  title     = {Enhancing federated learning in fog-aided IoT
by CPU frequency and wireless power control},
  journal   = {IEEE Internet Things
J.},
  volume    = 8,
  number    = 5,
  pages     = {3438–3445},
  month     = {Mar},
  year      = 2021,
}


%3
@inproceedings{mario8,
title = "Federated Learning over Wireless Networks: Optimization Model Design and Analysis",

author = "Tran, {Nguyen H.} and Wei Bao and Albert Zomaya and Nguyen, {Minh N.H.} and Hong, {Choong Seon}",
year = "2019",
month = apr,
doi = "10.1109/INFOCOM.2019.8737464",
language = "English",
series = "Proceedings - IEEE INFOCOM",
publisher = "Institute of Electrical and Electronics Engineers Inc.",
pages = "1387--1395",
booktitle = "INFOCOM 2019 - IEEE Conference on Computer Communications",
address = "United States",
}



@Article{mario9,
AUTHOR = {Rai, Sumit and Kumari, Arti and Prasad, Dilip K.},
TITLE = {Client Selection in Federated Learning under Imperfections in Environment},
JOURNAL = {AI},
VOLUME = {3},
YEAR = {2022},
NUMBER = {1},
PAGES = {124--145},
URL = {https://www.mdpi.com/2673-2688/3/1/8},
ISSN = {2673-2688},

DOI = {10.3390/ai3010008}
}



@article{mario10,
author = {Abdulrahman, Sawsan and Tout, Hanine and Mourad, Azzam and Talhi, Chamseddine},
year = {2020},
month = {10},
pages = {2327-4662},
title = {FedMCCS: Multicriteria Client Selection Model for Optimal IoT Federated Learning},
volume = {PP},
journal = {IEEE Internet of Things Journal},
doi = {10.1109/JIOT.2020.3028742}
}

@article{mario11,
 author = {Bonawitz, Keith and Eichner, Hubert and Grieskamp, Wolfgang and Huba, Dzmitry and Ingerman, Alex and Ivanov, Vladimir and Kiddon, Chloe and Konečný, Jakub and Mazzocchi, Stefano and McMahan, H. Brendan and Van Overveldt, Timon and Petrou, David and Ramage, Daniel and Roselander, Jason},
  

  title = {Towards Federated Learning at Scale: System Design},
publisher = {arXiv},
  
  year = {2019},
  booktitle	= {SysML 2019},
doi = {10.48550/ARXIV.1902.01046}}
}




@article{mario12,
  doi = {10.48550/ARXIV.1602.05629},
  
  url = {https://arxiv.org/abs/1602.05629},
  
  author = {McMahan, H. Brendan and Moore, Eider and Ramage, Daniel and Hampson, Seth and Arcas, Blaise Agüera y},
  
  keywords = {Machine Learning (cs.LG), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Communication-Efficient Learning of Deep Networks from Decentralized Data},
  
  publisher = {arXiv},
  
  year = {2017},
 publisher = {ARTIFICIAL INTELLIGENCE AND STATISTICS},
  
  year = {2017},
  volume={54},
  pages={1273-1282} 


}


@INPROCEEDINGS{mario14,
         author = {Laurila, J. K. and Gatica-Perez, Daniel and Aad, I. and J., Blom and Bornet, Olivier and Do, Trinh-Minh-Tri and Dousse, O. and Eberle, J. and Miettinen, M.},
       projects = {LS-CONTEXT},
          title = {The Mobile Data Challenge: Big Data for Mobile Computing Research},
      booktitle = {Pervasive Computing},
           year = {2012},
       location = {Newcastle},
            pdf = {https://publications.idiap.ch/attachments/papers/2012/Laurila_MDC_2012.pdf}
}

    


@article{marioo15,
 
  url = {https://github.com/arafeh94/localfed},
  

  title = {LocalFed}
}





@INPROCEEDINGS{mario13,
  author={Felter, Wes and Ferreira, Alexandre and Rajamony, Ram and Rubio, Juan},
  booktitle={2015 IEEE International Symposium on Performance Analysis of Systems and Software (ISPASS)}, 
  title={An updated performance comparison of virtual machines and Linux containers}, 
  year={2015},
  volume={},
  number={},
  pages={171-172},
  doi={10.1109/ISPASS.2015.7095802}}




@ARTICLE{mario16,  author={Abdulrahman, Sawsan and Tout, Hanine and Ould-Slimane, Hakima and Mourad, Azzam and Talhi, Chamseddine and Guizani, Mohsen},  journal={IEEE Internet of Things Journal},   title={A Survey on Federated Learning: The Journey From Centralized to Distributed On-Site Learning and Beyond},   year={2021},  volume={8},  number={7},  pages={5476-5497},  doi={10.1109/JIOT.2020.3030072}}

@INPROCEEDINGS{mario20,
  author={Zhang, Qin and Guo, Zhiwei and Yu, Keping and Al-Dulaimi, Anwer and Wei, Wei and Guizani, Mohsen},
  booktitle={2021 IEEE Global Communications Conference (GLOBECOM)}, 
  title={QoS-Aware Reliable Traffic Prediction Model Under Wireless Vehicular Networks}, 
  year={2021},
  volume={},
  number={},
  pages={1-6},
  doi={10.1109/GLOBECOM46510.2021.9685115}}

@ARTICLE{refbib1,
  author    = {C. T. Rim and D. Y. Hu and G. H. Cho},
  title     = {Transformers as Equivalent Circuits for Switches: General Proof and D-Q Transformation-Based Analysis},
  journal   = {IEEE Transactions on Industry Applications},
  volume    = 26,
  number    = 4,
  pages     = {832-840},
  month     = {July/August},
  year      = 1990,
}

@ARTICLE{refbib2,
  author    = {E. A. Vendruscolo and J. A. Pomilio},
  title     = {Motores de Indução Acionados por Inversores PWM-VSI: Estratégias para Atenuação de Sobretensões},
  journal   = {Eletrônica de Potência - SOBRAEP},
  volume    = 8,
  number    = 1,
  pages     = {49-56},
  month     = {Junho},
  year      = 2003,
}

@INPROCEEDINGS{refbib3,
  author    = "S. A. González and M. I. Valla and C. H. Muravchik",
  title     = "A Phase Modulated DGPS Transmitter Implemented with a CMRC",
  booktitle = "Proceedings of COBEP",
  volume    = 2,
  pages     = "553-558",
  year      = "2001"
}

@BOOK{refbib4,
  author    = {N. Mohan and T. M. Undeland and W. P. Robbins},
  title     = {Power Electronics: converters, applications, and design},
  publisher = {John Wiley \& Sons, Inc.},
  edition   = {2nd},
  address   = {New York, N.Y.},
  year      = {1995},
}

@misc{refbib5,
  author    = {T. A. Lipo and M. D. Manjrekar},
  title     = {Hybrid Topology for Multilevel Power Conversion},
  year      = {1999},
  month     =  "21~" # dec,
  note      = "{US} Patent 6 005 788",
}

@techreport{refbib6,
  author       = "\",
  title        = "IEEE Recommended Practices and Requirements for Harmonic Control in Electrical Power Systems",
  institution  = "IEEE Std. 519-1992",
  year         = "1993",
}

@misc{refbib7,
  author    = "{SW Technologies}",
  title     = "{SWDV Converter}",
  year      = "2001",
  url       = {www.sw.com.br},
  howpublished = "Online",
}

@phdthesis{refbib8,
  author    = {I. Barbi},
  title     = {Etude de Onduleurs Autoadaptifs Destines a la Alimentation de Machines Assynchrones},
  school    = {Institut National Polytechnique de Toulouse},
  year      = 1979,
  address   = {Toulouse, França},
}

@article{fedmll,
  Author = {He, Chaoyang and Li, Songze and So, Jinhyun and Zhang, Mi and Wang, Hongyi and Wang, Xiaoyang and Vepakomma, Praneeth and Singh, Abhishek and Qiu, Hang and Shen, Li and Zhao, Peilin and Kang, Yan and Liu, Yang and Raskar, Ramesh and Yang, Qiang and Annavaram, Murali and Avestimehr, Salman},
  Journal = {Advances in Neural Information Processing Systems, Best Paper Award at Federate Learning Workshop},
  Title = {FedML: A Research Library and Benchmark for Federated Machine Learning},
  Year = {2020}
}


@INPROCEEDINGS{mariofinals,
  author={Chahoud, Mario and Sami, Hani and Mourad, Azzam and Otrok, Hadi and Bentahar, Jamal and Guizani, Mohsen},
  booktitle={2023 International Wireless Communications and Mobile Computing (IWCMC)}, 
  title={Towards On-Demand Deployment of Multiple Clients and Heterogeneous Models in Federated Learning}, 
  year={2023},
  volume={},
  number={},
  pages={1556-1561},
  doi={10.1109/IWCMC58020.2023.10182555}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
@misc{paper1,
  doi = {10.48550/ARXIV.2207.09209},
  
  url = {https://arxiv.org/abs/2207.09209},
  
  author = {Zhang, Zaixi and Cao, Xiaoyu and Jia, Jinyuan and Gong, Neil Zhenqiang},
  
  keywords = {Cryptography and Security (cs.CR), Artificial Intelligence (cs.AI), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {FLDetector: Defending Federated Learning Against Model Poisoning Attacks via Detecting Malicious Clients},
  
  publisher = {arXiv},
  
  year = {2022},
  
  copyright = {Creative Commons Attribution Non Commercial Share Alike 4.0 International}
}

@INPROCEEDINGS{paper2,  author={Gu, Zhipin and Yang, Yuexiang},  booktitle={2021 IEEE International Parallel and Distributed Processing Symposium (IPDPS)},   title={Detecting Malicious Model Updates from Federated Learning on Conditional Variational Autoencoder},   year={2021},  volume={},  number={},  pages={671-680},  doi={10.1109/IPDPS49936.2021.00075}}


@unknown{paper3,
author = {Li, Suyi and Cheng, Yong and Wang, Wei and Liu, Yang and Chen, Tianjian},
year = {2020},
month = {02},
pages = {},
title = {Learning to Detect Malicious Clients for Robust Federated Learning}
}


@article{paper4,
author = {Zhou, Chuanxin and Sun, Yi and Wang, Degang and Gao, Qi and Tan, Zhiyuan},
title = {Fed-Fi: Federated Learning Malicious Model Detection Method Based on Feature Importance},
year = {2022},
issue_date = {2022},
publisher = {John Wiley \&amp; Sons, Inc.},
address = {USA},
volume = {2022},
issn = {1939-0114},
url = {https://doi.org/10.1155/2022/7268347},
doi = {10.1155/2022/7268347},
journal = {Sec. and Commun. Netw.},
month = {jan},
numpages = {11}
}

@unknown{paper5,
author = {Gâlvez, Rafa and Moonsamy, Veelasha and Diaz, Claudia},
year = {2020},
month = {07},
pages = {},
title = {Less is More: A privacy-respecting Android malware classifier using Federated Learning}
}

@misc{paper6,
  doi = {10.48550/ARXIV.2102.01854},
  
  url = {https://arxiv.org/abs/2102.01854},
  
  author = {Cao, Xiaoyu and Jia, Jinyuan and Gong, Neil Zhenqiang},
  
  keywords = {Cryptography and Security (cs.CR), Distributed, Parallel, and Cluster Computing (cs.DC), Machine Learning (cs.LG), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Provably Secure Federated Learning against Malicious Clients},
  
  publisher = {arXiv},
  
  year = {2021},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@unknown{paper7,
author = {Xu, Jian and Huang, Shao-Lun and Song, Linqi and Lan, Tian},
year = {2021},
month = {09},
pages = {},
title = {SignGuard: Byzantine-robust Federated Learning through Collaborative Malicious Gradient Filtering}
}


@inproceedings{paper8,
author = {Guo, Hanxi and Wang, Hao and Song, Tao and Hua, Yang and Lv, Zhangcheng and Jin, Xiulang and Xue, Zhengui and Ma, Ruhui and Guan, Haibing},
title = {Siren: Byzantine-Robust Federated Learning via Proactive Alarming},
year = {2021},
isbn = {9781450386388},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3472883.3486990},
doi = {10.1145/3472883.3486990},
booktitle = {Proceedings of the ACM Symposium on Cloud Computing},
pages = {47–60},
numpages = {14},
keywords = {Federated Learning, Byzantine-robust, Attack-agnostic Defense System},
location = {Seattle, WA, USA},
series = {SoCC '21}
}

@ARTICLE{paper9,  author={Zhang, Lefeng and Zhu, Tianqing and Xiong, Ping and Zhou, Wanlei and Yu, Philip},  journal={IEEE Transactions on Knowledge and Data Engineering},   title={A Robust Game-theoretical Federated Learning Framework with Joint Differential Privacy},   year={2022},  volume={},  number={},  pages={1-1},  doi={10.1109/TKDE.2021.3140131}}



@article{paper10,
author = {Rjoub, Gaith and Wahab, Omar and Bentahar, Jamal and Batineh, Ahmed},
year = {2022},
month = {04},
pages = {},
title = {Trust-driven Reinforcement Selection Strategy for Federated Learning on IoT Devices},
journal = {Computing},
doi = {10.1007/s00607-022-01078-1}
}

@article{paper11,
  title={A Game-Theoretic Approach for Robust Federated Learning},
  author={Esmaeel Tahanian and Mohammad Javad Amouei and Hadi Fateh and Mohsen Rezvani},
  journal={International Journal of Engineering},
  year={2021},
  volume={34},
  pages={832-842}
}

@article{paper12, title={FedInv: Byzantine-Robust Federated Learning by Inversing Local Model Updates}, volume={36}, url={https://ojs.aaai.org/index.php/AAAI/article/view/20903}, DOI={10.1609/aaai.v36i8.20903}, number={8}, journal={Proceedings of the AAAI Conference on Artificial Intelligence}, author={Zhao, Bo and Sun, Peng and Wang, Tao and Jiang, Keyu}, year={2022}, month={Jun.}, pages={9171-9179} }

@article{paper13,
title = {Federated against the cold: A trust-based federated learning approach to counter the cold start problem in recommendation systems},
journal = {Information Sciences},
volume = {601},
pages = {189-206},
year = {2022},
issn = {0020-0255},
doi = {https://doi.org/10.1016/j.ins.2022.04.027},
url = {https://www.sciencedirect.com/science/article/pii/S0020025522003632},
author = {Omar Abdel Wahab and Gaith Rjoub and Jamal Bentahar and Robin Cohen},
keywords = {Federated learning, Client selection, Recommendation system, Cold-start problem, Deep reinforcement learning, Trust establishment}
}

@ARTICLE{paper14,  author={Kang, Jiawen and Xiong, Zehui and Niyato, Dusit and Xie, Shengli and Zhang, Junshan},  journal={IEEE Internet of Things Journal},   title={Incentive Mechanism for Reliable Federated Learning: A Joint Optimization Approach to Combining Reputation and Contract Theory},   year={2019},  volume={6},  number={6},  pages={10700-10714},  doi={10.1109/JIOT.2019.2940820}}


@ARTICLE{paper15,  author={Kang, Jiawen and Xiong, Zehui and Niyato, Dusit and Zou, Yuze and Zhang, Yang and Guizani, Mohsen},  journal={IEEE Wireless Communications},   title={Reliable Federated Learning for Mobile Networks},   year={2020},  volume={27},  number={2},  pages={72-80},  doi={10.1109/MWC.001.1900119}}

@misc{paper16,
  doi = {10.48550/ARXIV.1910.04956},
  
  url = {https://arxiv.org/abs/1910.04956},
  
  author = {He, Chaoyang and Tan, Conghui and Tang, Hanlin and Qiu, Shuang and Liu, Ji},
  
  keywords = {Machine Learning (cs.LG), Social and Information Networks (cs.SI), Machine Learning (stat.ML), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Central Server Free Federated Learning over Single-sided Trust Social Networks},
  
  publisher = {arXiv},
  
  year = {2019},
  
  copyright = {Creative Commons Attribution 4.0 International}
}

@INPROCEEDINGS{paper17,  author={Wang, Guan and Dang, Charlie Xiaoqian and Zhou, Ziye},  booktitle={2019 IEEE International Conference on Big Data (Big Data)},   title={Measure Contribution of Participants in Federated Learning},   year={2019},  volume={},  number={},  pages={2597-2604},  doi={10.1109/BigData47090.2019.9006179}}

@inproceedings{paper18,
author = {Fang, Minghong and Cao, Xiaoyu and Jia, Jinyuan and Gong, Neil Zhenqiang},
title = {Local Model Poisoning Attacks to Byzantine-Robust Federated Learning},
year = {2020},
isbn = {978-1-939133-17-5},
publisher = {USENIX Association},
address = {USA},
booktitle = {Proceedings of the 29th USENIX Conference on Security Symposium},
articleno = {92},
numpages = {18},
series = {SEC'20}
}

@unknown{paper19,
author = {Muñoz-González, Luis and Co, Kenneth and Lupu, Emil},
year = {2019},
month = {09},
pages = {},
title = {Byzantine-Robust Federated Machine Learning through Adaptive Model Averaging}
}

@unknown{paper20,
author = {Li, Suyi and Cheng, Yong and Liu, Yang and Wang, Wei and Chen, Tianjian},
year = {2019},
month = {10},
pages = {},
title = {Abnormal Client Behavior Detection in Federated Learning}
}


@misc{paper21,
  doi = {10.48550/ARXIV.1808.04866},
  
  url = {https://arxiv.org/abs/1808.04866},
  
  author = {Fung, Clement and Yoon, Chris J. M. and Beschastnikh, Ivan},
  
  keywords = {Machine Learning (cs.LG), Cryptography and Security (cs.CR), Distributed, Parallel, and Cluster Computing (cs.DC), Machine Learning (stat.ML), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Mitigating Sybils in Federated Learning Poisoning},
  
  publisher = {arXiv},
  
  year = {2018},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}
@misc{paper23,
  doi = {10.48550/ARXIV.1807.00459},
  
  url = {https://arxiv.org/abs/1807.00459},
  
  author = {Bagdasaryan, Eugene and Veit, Andreas and Hua, Yiqing and Estrin, Deborah and Shmatikov, Vitaly},
  
  keywords = {Cryptography and Security (cs.CR), Machine Learning (cs.LG), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {How To Backdoor Federated Learning},
  
  publisher = {arXiv},
  
  year = {2018},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@misc{paper27,
  doi = {10.48550/ARXIV.1910.05467},
  
  url = {https://arxiv.org/abs/1910.05467},
  
  author = {Li, Zhaorui and Huang, Zhicong and Chen, Chaochao and Hong, Cheng},
  
  keywords = {Cryptography and Security (cs.CR), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Quantification of the Leakage in Federated Learning},
  
  publisher = {arXiv},
  
  year = {2019},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@inproceedings{paper24,
 author = {Blanchard, Peva and El Mhamdi, El Mahdi and Guerraoui, Rachid and Stainer, Julien},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {I. Guyon and U. Von Luxburg and S. Bengio and H. Wallach and R. Fergus and S. Vishwanathan and R. Garnett},
 pages = {},
 publisher = {Curran Associates, Inc.},
 title = {Machine Learning with Adversaries: Byzantine Tolerant Gradient Descent},
 url = {https://proceedings.neurips.cc/paper/2017/file/f4b9ec30ad9f68f89b29639786cb62ef-Paper.pdf},
 volume = {30},
 year = {2017}
}


@misc{paper25,
  doi = {10.48550/ARXIV.1811.12470},
  
  url = {https://arxiv.org/abs/1811.12470},
  
  author = {Bhagoji, Arjun Nitin and Chakraborty, Supriyo and Mittal, Prateek and Calo, Seraphin},
  
  keywords = {Machine Learning (cs.LG), Artificial Intelligence (cs.AI), Cryptography and Security (cs.CR), Machine Learning (stat.ML), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Analyzing Federated Learning through an Adversarial Lens},
  
  publisher = {arXiv},
  
  year = {2018},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@ARTICLE{paper26,  author={Rahman, Sawsan Abdul and Tout, Hanine and Talhi, Chamseddine and Mourad, Azzam},  journal={IEEE Network},   title={Internet of Things Intrusion Detection: Centralized, On-Device, or Federated Learning?},   year={2020},  volume={34},  number={6},  pages={310-317},  doi={10.1109/MNET.011.2000286}}


@article{paper28,
  title={Exploiting Unintended Feature Leakage in Collaborative Learning},
  author={Luca Melis and Congzheng Song and Emiliano De Cristofaro and Vitaly Shmatikov},
  journal={2019 IEEE Symposium on Security and Privacy (SP)},
  year={2019},
  pages={691-706}
}
@article{paper29,
author = {Geyer, Robin and Klein, Tassilo and Nabi, Moin},
year = {2017},
month = {12},
pages = {},
title = {Differentially Private Federated Learning: A Client Level Perspective}
}

@unknown{paper30,
author = {Agarwal, Naman and Suresh, Ananda and Yu, Felix and Kumar, Sanjiv and Mcmahan, H.},
year = {2018},
month = {05},
pages = {},
title = {cpSGD: Communication-efficient and differentially-private distributed SGD}
}

@misc{paper31,
  doi = {10.48550/ARXIV.1911.01812},
  
  url = {https://arxiv.org/abs/1911.01812},
  
  author = {Liu, Zaoxing and Li, Tian and Smith, Virginia and Sekar, Vyas},
  
  keywords = {Machine Learning (cs.LG), Cryptography and Security (cs.CR), Networking and Internet Architecture (cs.NI), Machine Learning (stat.ML), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Enhancing the Privacy of Federated Learning with Sketching},
  
  publisher = {arXiv},
  
  year = {2019},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@misc{paper32,
  doi = {10.48550/ARXIV.1711.10677},
  
  url = {https://arxiv.org/abs/1711.10677},
  
  author = {Hardy, Stephen and Henecka, Wilko and Ivey-Law, Hamish and Nock, Richard and Patrini, Giorgio and Smith, Guillaume and Thorne, Brian},
  
  keywords = {Machine Learning (cs.LG), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Private federated learning on vertically partitioned data via entity resolution and additively homomorphic encryption},
  
  publisher = {arXiv},
  
  year = {2017},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@inproceedings{paper33,
author = {Mandal, Kalikinkar and Gong, Guang},
year = {2019},
month = {11},
pages = {57-68},
title = {PrivFL: Practical Privacy-preserving Federated Regressions on High-dimensional Data over Mobile Networks},
isbn = {978-1-4503-6826-1},
doi = {10.1145/3338466.3358926}
}

@unknown{paper34,
author = {Feng, Yan and Yang, Xue and Fang, Weijun and Xia, Shu-Tao and Tang, Xiaohu},
year = {2020},
month = {02},
pages = {},
title = {Practical and Bilateral Privacy-preserving Federated Learning}
}

@inproceedings{paper35,
author = {Bonawitz, Keith and Ivanov, Vladimir and Kreuter, Ben and Marcedone, Antonio and McMahan, H. Brendan and Patel, Sarvar and Ramage, Daniel and Segal, Aaron and Seth, Karn},
title = {Practical Secure Aggregation for Privacy-Preserving Machine Learning},
year = {2017},
isbn = {9781450349468},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3133956.3133982},
doi = {10.1145/3133956.3133982},
booktitle = {Proceedings of the 2017 ACM SIGSAC Conference on Computer and Communications Security},
pages = {1175–1191},
numpages = {17},
keywords = {federated learning, machine learning, secure aggregation, privacy-preserving protocols},
location = {Dallas, Texas, USA},
series = {CCS '17}
}

@inproceedings{paper36,
title	= {Practical Secure Aggregation for Federated Learning on User-Held Data},
author	= {K. A. Bonawitz and Vladimir Ivanov and Ben Kreuter and Antonio Marcedone and H. Brendan McMahan and Sarvar Patel and Daniel Ramage and Aaron Segal and Karn Seth},
year	= {2016},
URL	= {https://arxiv.org/abs/1611.04482},
booktitle	= {NIPS Workshop on Private Multi-Party Machine Learning}
}

@misc{paper37,
  doi = {10.48550/ARXIV.1911.02254},
  
  url = {https://arxiv.org/abs/1911.02254},
  
  author = {Niu, Chaoyue and Wu, Fan and Tang, Shaojie and Hua, Lifeng and Jia, Rongfei and Lv, Chengfei and Wu, Zhihua and Chen, Guihai},
  
  keywords = {Machine Learning (cs.LG), Cryptography and Security (cs.CR), Distributed, Parallel, and Cluster Computing (cs.DC), Machine Learning (stat.ML), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Secure Federated Submodel Learning},
  
  publisher = {arXiv},
  
  year = {2019},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@inproceedings{paper38,
author = {Truex, Stacey and Baracaldo, Nathalie and Anwar, Ali and Steinke, Thomas and Ludwig, Heiko and Zhang, Rui and Zhou, Yi},
title = {A Hybrid Approach to Privacy-Preserving Federated Learning},
year = {2019},
isbn = {9781450368339},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3338501.3357370},
doi = {10.1145/3338501.3357370},
booktitle = {Proceedings of the 12th ACM Workshop on Artificial Intelligence and Security},
pages = {1–11},
numpages = {11},
keywords = {differential privacy, secure multiparty computation, federated learning, privacy, privacy-preserving machine learning},
location = {London, United Kingdom},
series = {AISec'19}
}

@ARTICLE{paper39,  author={Kim, Hyesung and Park, Jihong and Bennis, Mehdi and Kim, Seong-Lyun},  journal={IEEE Communications Letters},   title={Blockchained On-Device Federated Learning},   year={2020},  volume={24},  number={6},  pages={1279-1283},  doi={10.1109/LCOMM.2019.2921755}}

@article{paper41,
  title={Privacy-preserving Heterogeneous Federated Transfer Learning},
  author={Dashan Gao and Yang Liu and Anbu Huang and Ce Ju and Han Yu and Qiang Yang},
  journal={2019 IEEE International Conference on Big Data (Big Data)},
  year={2019},
  pages={2552-2559}
}

@INPROCEEDINGS{task2first,  author={Bhuyan, Neelkamal and Moharir, Sharayu},  booktitle={2022 14th International Conference on COMmunication Systems \& NETworkS (COMSNETS)},   title={Multi-Model Federated Learning},   year={2022},  volume={},  number={},  pages={779-783},  doi={10.1109/COMSNETS53615.2022.9668435}}

@article{task2second,
author = {Long, Guodong and Xie, Ming and Shen, Tao and Zhou, Tianyi and Wang, Xianzhi and Jiang, Jing},
year = {2022},
month = {06},
pages = {1-20},
title = {Multi-center federated learning: clients clustering for better personalization},
journal = {World Wide Web},
doi = {10.1007/s11280-022-01046-x}
}



@article{mario1kk,
title = {On the feasibility of Federated Learning towards on-demand client deployment at the edge},
journal = {Information Processing \& Management},
volume = {60},
number = {1},
pages = {103150},
year = {2023},
issn = {0306-4573},
doi = {https://doi.org/10.1016/j.ipm.2022.103150},
url = {https://www.sciencedirect.com/science/article/pii/S0306457322002515},
author = {Mario Chahoud and Safa Otoum and Azzam Mourad},
}


@ARTICLE{hani1,  author={Sami, Hani and Mourad, Azzam},  journal={IEEE Transactions on Network and Service Management},   title={Dynamic On-Demand Fog Formation Offering On-the-Fly IoT Service Deployment},   year={2020},  volume={17},  number={2},  pages={1026-1039},  doi={10.1109/TNSM.2019.2963643}}



@ARTICLE{hani2,  author={Sami, Hani and Mourad, Azzam and El-Hajj, Wassim},  journal={IEEE/ACM Transactions on Networking},   title={Vehicular-OBUs-As-On-Demand-Fogs: Resource and Context Aware Deployment of Containerized Micro-Services},   year={2020},  volume={28},  number={2},  pages={778-790},  doi={10.1109/TNET.2020.2973800}}


@INPROCEEDINGS{sssss,
  author={Chahoud, Mario and Mourad, Azzam and Otrok, Hadi and Guizani, Mohsen},
  booktitle={IEEE INFOCOM 2023 - IEEE Conference on Computer Communications Workshops (INFOCOM WKSHPS)}, 
  title={Towards Trust Driven On-Demand Client Deployment in Federated Learning}, 
  year={2023},
  volume={},
  number={},
  pages={1-6},
  doi={10.1109/INFOCOMWKSHPS57453.2023.10225756}}


@misc{lit1,
  doi = {10.48550/ARXIV.2207.09209},
  
  url = {https://arxiv.org/abs/2207.09209},
  
  author = {Zhang, Zaixi and Cao, Xiaoyu and Jia, Jinyuan and Gong, Neil Zhenqiang},
  
  keywords = {Cryptography and Security (cs.CR), Artificial Intelligence (cs.AI), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {FLDetector: Defending Federated Learning Against Model Poisoning Attacks via Detecting Malicious Clients},
  
  publisher = {arXiv},
  
  year = {2022},
  
  copyright = {Creative Commons Attribution Non Commercial Share Alike 4.0 International}
}


@INPROCEEDINGS{lit2,  author={Gu, Zhipin and Yang, Yuexiang},  booktitle={2021 IEEE International Parallel and Distributed Processing Symposium (IPDPS)},   title={Detecting Malicious Model Updates from Federated Learning on Conditional Variational Autoencoder},   year={2021},  volume={},  number={},  pages={671-680},  doi={10.1109/IPDPS49936.2021.00075}}

@article{lit5,
  title={A Game-Theoretic Approach for Robust Federated Learning},
  author={Esmaeel Tahanian and Mohammad Javad Amouei and Hadi Fateh and Mohsen Rezvani},
  journal={International Journal of Engineering},
  year={2021},
  volume={34},
  pages={832-842}
}



@article{lit3,
author = {Zhou, Chuanxin and Sun, Yi and Wang, Degang and Gao, Qi and Tan, Zhiyuan},
title = {Fed-Fi: Federated Learning Malicious Model Detection Method Based on Feature Importance},
year = {2022},
issue_date = {2022},
publisher = {John Wiley \&amp; Sons, Inc.},
address = {USA},
volume = {2022},
issn = {1939-0114},
url = {https://doi.org/10.1155/2022/7268347},
doi = {10.1155/2022/7268347},
journal = {Sec. and Commun. Netw.},
month = {jan},
numpages = {11}
}

@unknown{lit4,
author = {Xu, Jian and Huang, Shao-Lun and Song, Linqi and Lan, Tian},
year = {2021},
month = {09},
pages = {},
title = {SignGuard: Byzantine-robust Federated Learning through Collaborative Malicious Gradient Filtering}
}


@article{lit6, title={FedInv: Byzantine-Robust Federated Learning by Inversing Local Model Updates}, volume={36}, url={https://ojs.aaai.org/index.php/AAAI/article/view/20903}, DOI={10.1609/aaai.v36i8.20903}, number={8}, journal={Proceedings of the AAAI Conference on Artificial Intelligence}, author={Zhao, Bo and Sun, Peng and Wang, Tao and Jiang, Keyu}, year={2022}, month={Jun.}, pages={9171-9179} }


@article{lit7,
author = {Rjoub, Gaith and Wahab, Omar and Bentahar, Jamal and Batineh, Ahmed},
year = {2022},
month = {04},
pages = {},
title = {Trust-driven Reinforcement Selection Strategy for Federated Learning on IoT Devices},
journal = {Computing},
doi = {10.1007/s00607-022-01078-1}
}


@article{lit8,
title = {Federated against the cold: A trust-based federated learning approach to counter the cold start problem in recommendation systems},
journal = {Information Sciences},
volume = {601},
pages = {189-206},
year = {2022},
issn = {0020-0255},
doi = {https://doi.org/10.1016/j.ins.2022.04.027},
url = {https://www.sciencedirect.com/science/article/pii/S0020025522003632},
author = {Omar Abdel Wahab and Gaith Rjoub and Jamal Bentahar and Robin Cohen},
keywords = {Federated learning, Client selection, Recommendation system, Cold-start problem, Deep reinforcement learning, Trust establishment}
}


@misc{lit9,
  doi = {10.48550/ARXIV.1910.04956},
  
  url = {https://arxiv.org/abs/1910.04956},
  
  author = {He, Chaoyang and Tan, Conghui and Tang, Hanlin and Qiu, Shuang and Liu, Ji},
  
  keywords = {Machine Learning (cs.LG), Social and Information Networks (cs.SI), Machine Learning (stat.ML), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Central Server Free Federated Learning over Single-sided Trust Social Networks},
  
  publisher = {arXiv},
  
  year = {2019},
  
  copyright = {Creative Commons Attribution 4.0 International}
}


@unknown{lit10,
author = {Muñoz-González, Luis and Co, Kenneth and Lupu, Emil},
year = {2019},
month = {09},
pages = {},
title = {Byzantine-Robust Federated Machine Learning through Adaptive Model Averaging}
}

@inproceedings{defaultfl,
  author    = {Brendan McMahan and
               Eider Moore and
               Daniel Ramage and
               Seth Hampson and
               Blaise Ag{\"{u}}era y Arcas},
  editor    = {Aarti Singh and
               Xiaojin (Jerry) Zhu},
  title     = {Communication-Efficient Learning of Deep Networks from Decentralized
               Data},
  booktitle = {Proceedings of the 20th International Conference on Artificial Intelligence
               and Statistics, {AISTATS} 2017, 20-22 April 2017, Fort Lauderdale,
               FL, {USA}},
  series    = {Proceedings of Machine Learning Research},
  volume    = {54},
  pages     = {1273--1282},
  publisher = {{PMLR}},
  year      = {2017},
  url       = {http://proceedings.mlr.press/v54/mcmahan17a.html},
  timestamp = {Wed, 29 May 2019 08:41:44 +0200},
  biburl    = {https://dblp.org/rec/conf/aistats/McMahanMRHA17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@INPROCEEDINGS{cluster,
  author={Sami, Hani and Mourad, Azzam},
  booktitle={2018 International Conference on Computational Science and Computational Intelligence (CSCI)}, 
  title={Towards Dynamic On-Demand Fog Computing Formation Based On Containerization Technology}, 
  year={2018},
  volume={},
  number={},
  pages={960-965},
  doi={10.1109/CSCI46756.2018.00187}}



@ARTICLE{firstpaperr,
  author={Chahoud, Mario and Sami, Hani and Mourad, Azzam and Otoum, Safa and Otrok, Hadi and Bentahar, Jamal and Guizani, Mohsen},
  journal={IEEE Internet of Things Journal}, 
  title={ON-DEMAND-FL: A Dynamic and Efficient Multi-Criteria Federated Learning Client Deployment Scheme}, 
  year={2023},
  volume={},
  number={},
  pages={1-1},
  doi={10.1109/JIOT.2023.3265564}}


  @article{secondfirstpaperr,
title = {On the feasibility of Federated Learning towards on-demand client deployment at the edge},
journal = {Information Processing \& Management},
volume = {60},
number = {1},
pages = {103150},
year = {2023},
issn = {0306-4573},
doi = {https://doi.org/10.1016/j.ipm.2022.103150},
url = {https://www.sciencedirect.com/science/article/pii/S0306457322002515},
author = {Mario Chahoud and Safa Otoum and Azzam Mourad}
}


@article{arafehlocalfedd,
title = {ModularFed: Leveraging modularity in federated learning frameworks},
journal = {Internet of Things},
volume = {22},
pages = {100694},
year = {2023},
issn = {2542-6605},
doi = {https://doi.org/10.1016/j.iot.2023.100694},
url = {https://www.sciencedirect.com/science/article/pii/S2542660523000173},
author = {Mohamad Arafeh and Hadi Otrok and Hakima Ould-Slimane and Azzam Mourad and Chamseddine Talhi and Ernesto Damiani}
}

@article{proveclustering,
author = {Lim, Wei Yang Bryan and Nguyen, Cong and Dinh Thai, Hoang and Jiao, Yutao and Liang, Ying-Chang and Yang, Qiang and Niyato, Dusit and Miao, Chunyan},
year = {2020},
month = {04},
pages = {1-1},
title = {Federated Learning in Mobile Edge Networks: A Comprehensive Survey},
volume = {PP},
journal = {IEEE Communications Surveys \& Tutorials},
doi = {10.1109/COMST.2020.2986024}
}
@ARTICLE{proveclsutering2,
  author={Chen, Yiqiang and Qin, Xin and Wang, Jindong and Yu, Chaohui and Gao, Wen},
  journal={IEEE Intelligent Systems}, 
  title={FedHealth: A Federated Transfer Learning Framework for Wearable Healthcare}, 
  year={2020},
  volume={35},
  number={4},
  pages={83-93},
  doi={10.1109/MIS.2020.2988604}}


  @article{multiarea1,
title = {New data preprocessing trends based on ensemble of multiple preprocessing techniques},
journal = {TrAC Trends in Analytical Chemistry},
volume = {132},
pages = {116045},
year = {2020},
issn = {0165-9936},
doi = {https://doi.org/10.1016/j.trac.2020.116045},
url = {https://www.sciencedirect.com/science/article/pii/S0165993620302740},
author = {Puneet Mishra and Alessandra Biancolillo and Jean Michel Roger and Federico Marini and Douglas N. Rutledge}
}

@article{multiarea2,
title = {A novel image-based transfer learning framework for cross-domain HVAC fault diagnosis: From multi-source data integration to knowledge sharing strategies},
journal = {Energy and Buildings},
volume = {262},
pages = {111995},
year = {2022},
issn = {0378-7788},
doi = {https://doi.org/10.1016/j.enbuild.2022.111995},
url = {https://www.sciencedirect.com/science/article/pii/S0378778822001669},
author = {Cheng Fan and Weilin He and Yichen Liu and Peng Xue and Yangping Zhao}
}

@ARTICLE{form1,
  author={Wei, Lijun and Wu, Jing and Long, Chengnian and Li, Bo},
  journal={IEEE Internet of Things Journal}, 
  title={On Designing Context-Aware Trust Model and Service Delegation for Social Internet of Things}, 
  year={2021},
  volume={8},
  number={6},
  pages={4775-4787},
  doi={10.1109/JIOT.2020.3028380}}

  @misc{form2,
title	= {Federated Learning for Mobile Keyboard Prediction},
author	= {Andrew Hard and Chloé M Kiddon and Daniel R Ramage and Françoise Simone Beaufays and Hubert Eichner and Kanishka Rao and Rajiv Mathews and Sean Augenstein and Swaroop Ramaswamy},
year	= {2019}
}


@article{form3,
title = {An energy-efficient artificial bee colony-based clustering in the internet of things},
journal = {Computers \& Electrical Engineering},
volume = {86},
pages = {106733},
year = {2020},
issn = {0045-7906},
doi = {https://doi.org/10.1016/j.compeleceng.2020.106733},
url = {https://www.sciencedirect.com/science/article/pii/S0045790620305887},
author = {Shamim Yousefi and Farnaz Derakhshan and Hadi S. Aghdasi and Hadis Karimipour}
}

@article{form4,
title = {Privacy-preserving Byzantine-robust federated learning},
journal = {Computer Standards \& Interfaces},
volume = {80},
pages = {103561},
year = {2022},
issn = {0920-5489},
doi = {https://doi.org/10.1016/j.csi.2021.103561},
url = {https://www.sciencedirect.com/science/article/pii/S0920548921000568},
author = {Xu Ma and Yuqing Zhou and Laihua Wang and Meixia Miao}
}

@book{inalgo,
  title={How to detect and handle outliers},
  author={Iglewicz, Boris and Hoaglin, David Caster},
  volume={16},
  year={1993},
  publisher={Asq Press}
}

@ARTICLE{form5,
  author={Taïk, Afaf and Mlika, Zoubeir and Cherkaoui, Soumaya},
  journal={IEEE Transactions on Intelligent Transportation Systems}, 
  title={Clustered Vehicular Federated Learning: Process and Optimization}, 
  year={2022},
  volume={23},
  number={12},
  pages={25371-25383},
  doi={10.1109/TITS.2022.3149860}}

  @article{form6,
title = {Revisiting agglomerative clustering},
journal = {Physica A: Statistical Mechanics and its Applications},
volume = {585},
pages = {126433},
year = {2022},
issn = {0378-4371},
doi = {https://doi.org/10.1016/j.physa.2021.126433},
url = {https://www.sciencedirect.com/science/article/pii/S0378437121007068},
author = {Eric K. Tokuda and Cesar H. Comin and Luciano da F. Costa}
}

@misc{osamaboost,
      title={FedMint: Intelligent Bilateral Client Selection in Federated Learning with Newcomer IoT Devices}, 
      author={Osama Wehbi and Sarhad Arisdakessian and Omar Abdel Wahab and Hadi Otrok and Safa Otoum and Azzam Mourad and Mohsen Guizani},
      year={2022},
      eprint={2211.01805},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@article{bosstr,
title = {An endorsement-based trust bootstrapping approach for newcomer cloud services},
journal = {Information Sciences},
volume = {527},
pages = {159-175},
year = {2020},
issn = {0020-0255},
doi = {https://doi.org/10.1016/j.ins.2020.03.102},
url = {https://www.sciencedirect.com/science/article/pii/S0020025520302838},
author = {Omar Abdel Wahab and Robin Cohen and Jamal Bentahar and Hadi Otrok and Azzam Mourad and Gaith Rjoub}
}

@inproceedings{reftostd,
  title={Learning with continuous classes},
  author={Quinlan, John R and others},
  booktitle={5th Australian joint conference on artificial intelligence},
  volume={92},
  pages={343--348},
  year={1992},
  organization={World Scientific}
}


@ARTICLE{hammoudpap,
  author={Hammoud, Ahmad and Otrok, Hadi and Mourad, Azzam and Dziong, Zbigniew},
  journal={IEEE Transactions on Network and Service Management}, 
  title={On Demand Fog Federations for Horizontal Federated Learning in IoV}, 
  year={2022},
  volume={19},
  number={3},
  pages={3062-3075},
  doi={10.1109/TNSM.2022.3172370}}


  @ARTICLE{wazz,
  author={Wazzeh, Mohamad and Ould-Slimane, Hakima and Talhi, Chamseddine and Mourad, Azzam and Guizani, Mohsen},
  journal={IEEE Network}, 
  title={Privacy-Preserving Continuous Authentication for Mobile and IoT Systems Using Warmup-Based Federated Learning}, 
  year={2022},
  volume={},
  number={},
  pages={1-7},
  doi={10.1109/MNET.121.2200099}}



@ARTICLE{newtointro1,
  author={Hu, Fei and Zhou, Wuneng and Liao, Kaili and Li, Hongliang and Tong, Dongbing},
  journal={IEEE Internet of Things Journal}, 
  title={Towards Federated Learning Models Resistant to Adversarial Attacks}, 
  year={2023},
  volume={},
  number={},
  pages={1-1},
  doi={10.1109/JIOT.2023.3272334}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@article{mna1,
title = {Leveraging heuristic client selection for enhanced secure federated submodel learning},
journal = {Information Processing \& Management},
volume = {60},
number = {3},
pages = {103211},
year = {2023},
issn = {0306-4573},
doi = {https://doi.org/10.1016/j.ipm.2022.103211},
url = {https://www.sciencedirect.com/science/article/pii/S0306457322003120},
author = {Panyu Liu and Tongqing Zhou and Zhiping Cai and Fang Liu and Yeting Guo}}
}


@INPROCEEDINGS{basedconference,
  author={Chahoud, Mario and Mourad, Azzam and Otrok, Hadi and Guizani, Mohsen},
  booktitle={IEEE INFOCOM 2023 - IEEE Conference on Computer Communications Workshops (INFOCOM WKSHPS)}, 
  title={Towards Trust Driven On-Demand Client Deployment in Federated Learning}, 
  year={2023},
  volume={},
  number={},
  pages={1-6},
  keywords={Toxicology;Federated learning;Conferences;Computer architecture;Containers;Data models;Reliability;On-Demand;Trust;Malicious Clients;Volun-teering Devices;Containerization Technology;Federated Learning;Client Selection},
  doi={10.1109/INFOCOMWKSHPS57453.2023.10225756}}
